Age-Dependent Differential Privacy

The proliferation of real-time applications has motivated extensive research on analyzing and optimizing data freshness in the context of \textit{age of information}. However, classical frameworks of privacy (e.g., differential privacy (DP)) have overlooked the impact of data freshness on privacy guarantees, which may lead to unnecessary accuracy loss when trying to achieve meaningful privacy guarantees in time-varying databases. In this work, we introduce \textit{age-dependent DP}, taking into account the underlying stochastic nature of a time-varying database. In this new framework, we establish a connection between classical DP and age-dependent DP, based on which we characterize the impact of data staleness and temporal correlation on privacy guarantees. Our characterization demonstrates that \textit{aging}, i.e., using stale data inputs and/or postponing the release of outputs, can be a new strategy to protect data privacy in addition to noise injection in the traditional DP framework. Furthermore, to generalize our results to a multi-query scenario, we present a sequential composition result for age-dependent DP under any publishing and aging policies. We then characterize the optimal tradeoffs between privacy risk and utility and show how this can be achieved. Finally, case studies show that to achieve a target of an arbitrarily small privacy risk in a single-query case, combing aging and noise injection only leads to a bounded accuracy loss, whereas using noise injection only (as in the benchmark case of DP) will lead to an unbounded accuracy loss.

==> [TIT 23] Age-Dependent DP-2/Reference.tex <==

\bibliographystyle{ACM-Reference-Format}
% \bibliography{sample-base}


	\begin{thebibliography}{99}

\bibitem{Sigmetrics}
M. Zhang, E. Wei, R. Berry, and J. Huang, ``Age-dependent differential privacy'', \textit{ACM Sigmetrics/IFIP PERFORMANCE}, pp. 115-116, June 2022.

\bibitem{AoIsurvey}
R. D. Yates,  Y. Sun, D. R.Brown, S. K. Kaul, E. Modiano, and S. Ulukus,  ``Age of information: An introduction and survey,'' \textit{IEEE Journal on Selected Areas in Communications}, vol. 39, no. 5, pp. 1183-1210, 2021.

\bibitem{DP}
C. Dwork, ``Differential privacy,''  \textit{Proc. 33rd International Colloquium on Automata, Languages and Programming, part II (ICALP 2006)}, vol. 4052, pp. 1–12, Venice, Italy, July 2006.

% \bibitem{}

\bibitem{Aapl}
Differential Privacy Team Apple, Learning with privacy at scale. Technical report, Apple, 2017.

\bibitem{Goog}
Ú. Erlingsson, V. Pihur, and A. Korolova, ``Rappor: Randomized aggregatable privacy-preserving ordinal response,'' \textit{in Proc. ACM SIGSAC Conf. Comput. Commun. Sec. (CCS)}, pp. 1054–1067, 2014.

\bibitem{Census}
J. M. Abowd, ``The challenge of scientific reproducibility and privacy protection for statistical agencies,'' Census Scientific Advisory Committee, 2016.

\bibitem{Msft}
B. Ding, J. Kulkarni, and S. Yekhanin, ``Collecting telemetry data privately,'' \textit{in Proc. Advances in Neural Information Processing Systems (NIPS)}, 2017.


\bibitem{Anonymity}
P. Samarati and L. Sweeney, ``Generalizing data to provide anonymity when disclosing information,'' in \textit{Proc. ACM SIGACT-SIGMOD-SIGART Symposium on Principles of Database Systems (PODS)}, Seattle, WA, USA, 1998.

\bibitem{Closeness}
N. Li, Tiancheng Li, and S. Venkatasubramanian, ``t-Closeness: Privacy beyond k-anonymity and l-diversity,'' in \textit{Proc. IEEE Int. Conf. Data Engineering (ICDE’)}, IEEE, 106–115.


\bibitem{Location}
R. Shokri,  G. Theodorakopoulos, J. Y. Le Boudec, and J. P. Hubaux,  ``Quantifying location privacy,'' in \textit{Proc. 2011 IEEE symposium on security and privacy (pp. 247-262)}, 2011, May.

\bibitem{SmartMeter}
I. Rouf, H Mustafa, M. Xu, W. Xu, R. Miller, and M. Gruteser,  ``Neighborhood watch: Security and privacy analysis of automatic meter reading systems,'' in \textit{Proc. ACM Conf Comput. Commun. Sec.}, pp. 462-473, 2012, October.

\bibitem{Survey}
I. Wagner and D. Eckhoff,  ``Technical privacy metrics: a systematic survey,'' ACM Computing Surveys (CSUR), 51(3), pp.1-38, 2018.
	
\bibitem{RDP}
R. Hall, A. Rinaldo, and L. Wasserman, ``Random differential privacy,''  2011. ArXiv preprint: 1112.2680.

\bibitem{BDP1}
B. Yang, I. Sato,  and H. Nakagawa, ``Bayesian differential privacy on correlated data,'' \textit{in Proc. ACM SIGMOD international conference on Management of Data,} pp. 747-762, May 2015.

\bibitem{BDP2}
A. Triastcyn  and B. Faltings, ``Bayesian differential privacy for machine learning,'' \textit{in International Conf. Machine Learning (PMLR),}  (pp. 9583-9592). 2020, November. 
	
\bibitem{Pufferfish}	
	D. Kifer and A. Machanavajjhala, ``Pufferfish: A framework for mathematical privacy definitions,'' \textit{ACM Trans. Database Syst.}, vol. 39, no. 1, pp. 3-36, Jan. 2014.
	
\bibitem{Pufferfish2}	
S. Song, Y. Wang, and K. Chaudhuri,  ``Pufferfish privacy mechanisms for correlated data,'' \textit{in Proc. the 2017 ACM International Conference on Management of Data (SIGMOD '17)}, New York, NY, USA, 1291–1306, 2017.
	
\bibitem{Dwork2}	
C. Dwork, M. Naor, T. Pitassi, and G. N. Rothblum, ``Differential privacy under continual observation,'' in \textit{Proc. ACM symposium on Theory of computing (STOC)}, pp. 715-724, June 2010.
	
\bibitem{Static1}	
A. Blum, K. Ligett, and A. Roth, ``A learning theory approach to non-interactive database privacy,'' in \textit{Proc. ACM symposium on Theory of computing (STOC)},  pp. 609–618, 2008.
	
\bibitem{Static2}
M. Hardt and G. N. Rothblum. ``A multiplicative weights mechanism for privacy-preserving data analysis,'' \textit{in Proc. IEEE Symposium on Foundations of Computer Science (FOCS)}, pp. 61–70, 2010.

\bibitem{Dwork3}
C. Dwork, V. Feldman, M. Hardt, T. Pitassi, O. Reingold, and A. Roth, ``The reusable holdout: Preserving validity in adaptive data analysis,'' \textit{Science}, vol. 349, no. 6248, pp: 636–638, 2015.


\bibitem{Growing1}		
A. Smith and A. G. Thakurta, ``(Nearly) optimal algorithms for private online learning in full information and bandit settings,'' \textit{in Proc. Advances in Neural Information Processing Systems (NIPS)}, pp. 2733—2741, 2013.
	
\bibitem{Growing2}		
T.-H. H. Chan, E. Shi, and D. Song, ``Private and continual release of statistics,'' \textit{ACM Trans. Info. Syst. Sec.}, 14(3):26, 2011.
	
\bibitem{Growing3}	
R. Cummings, S. Krehbiel, K. A. Lai, and U. Tantipongpipat, ``Differential privacy for growing databases,'' in \textit{Advances in Neural Information Processing Systems}, pp. 8864–8873, 2018.
	
\bibitem{Discounted}
F. Farokhi,  ``Temporally discounted differential privacy for evolving datasets on an infinite horizon,'' in \textit{Proc. ACM/IEEE International Conference on Cyber-Physical Systems (ICCPS)}, 2020.
	
	
\bibitem{TimeCorrelation}
Y. Cao, M. Yoshikawa, Y. Xiao and L. Xiong, ``Quantifying differential privacy in continuous data release under temporal correlations,'' in \textit{IEEE Transactions on Knowledge and Data Engineering}, vol. 31, no. 7, pp. 1281-1295, 1 July 2019.

\bibitem{TimeConfuse}
B. Hoh, M. Gruteser, H. Xiong, and A. Alrabady, ``Preserving privacy in GPS traces via uncertainty-aware path cloaking,'' in \textit{Proc. ACM conference on Computer and communications security (CCS)}. New York, NY, USA, 161–171. 2007.


\bibitem{TimeSuccess}
M. Wright, M. Adler, B. N. Levine, and C. Shields, ``An analysis of the degradation of anonymous protocols,'' in \textit{Proc. Network and Distributed System Security Symp. (NDSS'02)}, Vol. 2. 39–50, 2002.

\bibitem{TrackTime}
K. Sampigethaya, L. Huang, M. Li, R. Poovendran, K. Matsuura, and K. Sezaki, ``ARAVAN: Providing location privacy for VANET,'' \textit{in Embedded Security in Cars (ESCAR’05)}. 29–37, 2005.

\bibitem{AoI0}
R. D. Yates and S. K. Kaul, ``The age of information: Real-time status updating by multiple sources,'' \textit{IEEE Trans. Inf. Theory}, vol. 65, no. 3, pp. 1807–1827, Mar. 2019.		
		
\bibitem{AoI1}
		Q. He, D. Yuan, and A. Ephremides, ``Optimal link scheduling for age minimization in wireless systems,'' \textit{IEEE Trans. Inf. Theory}, vol. 64, no. 7, pp. 5381-5394, July 2018.

% 		\bibitem{AoI42}
% 		Q. He, D. Yuan, and A. Ephremides, ``On optimal link scheduling with min-max peak age of information in wireless systems,” in \textit{Proc. IEEE Int. Commun. Conf. (ICC)}, 2016.
		
% 		\bibitem{AoI5}
% 		I. Kadota, E. Uysal-Biyikoglu, R. Singh, and E. Modiano, ``Minimizing the age of information in broadcast wireless networks,” in  \textit{Proc. 54th Ann. Allerton Conf. Commun. Contr. Comput.}, 2016.
		
		\bibitem{AoI2}
		C. Kam, S. Kompella, and A. Ephremides, ``Age of information under random updates,'' in \textit{Proc. IEEE Int. Symp. Inf. Theory (ISIT)},  2013.
		
		\bibitem{AoI3}
		Y. Sun, E. Uysal-Biyikoglu, R. D. Yates, C. E. Koksal, and N. B. Shroff, ``Update or wait: How to keep your data fresh,'' \textit{IEEE Trans. Inf. Theory}, vol. 63, no. 11, pp. 7492-7508, Nov.  2017.
		
		\bibitem{AoI4}
		A. M. Bedewy, Y. Sun, S. Kompella, N. B. Shroff, ``Optimal sampling and scheduling for timely status updates in multi-source networks,'' \textit{IEEE Trans. Inf. Theory}, vol. 67, no. 6, pp. 4019-4034, June 2021
		
		\bibitem{AoI5}
	R. Talak, S. Karaman and E. Modiano, ``Optimizing Information Freshness in Wireless Networks Under General Interference Constraints,'' in \textit{IEEE/ACM Trans. Netw.}, vol. 28, no. 1, pp. 15-28, Feb. 2020
		
		\bibitem{AoI6}
		I. Kadota, A. Sinha and E. Modiano, ``Scheduling Algorithms for Optimizing Age of Information in Wireless Networks With Throughput Constraints,'' in \textit{IEEE/ACM Trans. Netw.}, vol. 27, no. 4, pp. 1359-1372, Aug. 2019.
		
\bibitem{AoI7}
Y. Sun and B. Cyr,  ``Sampling for data freshness optimization: Non-linear age functions,'' \textit{J. Commun. Netw.}, vol. 21, no. 3, pp. 204-219, 2019.

		
\bibitem{AoI8}
M. Zhang, A. Arafa, J. Huang and H. V. Poor, ``Pricing Fresh Data,''  \textit{IEEE Journal on Selected Areas in Communications}, vol. 39, no. 5, pp. 1211-1225, May 2021.

		
\bibitem{AoI9}
M. Zhang, A. Arafa, E. Wei and R. Berry, ``Optimal and Quantized Mechanism Design for Fresh Data Acquisition," \textit{IEEE Journal on Selected Areas in Communications},  vol. 39, no. 5, pp. 1226-1239, May 2021.

\bibitem{AoIPrivacy}
R. Jin, X. He and H. Dai, ``Minimizing the Age of Information in the Presence of Location Privacy-Aware Mobile Agents,'' \textit{IEEE Trans. Commun.}, vol. 69, no. 2, pp. 1053-1067, Feb. 2021.

\bibitem{composition}
P. Kairouz, S. Oh, and P. Viswanath,  ``The composition theorem for differential privacy,'' in International conference on machine learning, pp. 1376-1385, \textit{PMLR},  2015.

\bibitem{Markov}
D. A. Levin  and Y. Peres. ``Markov chains and mixing times,'' vol. 107. \textit{American Mathematical Soc.}, 2017.

\bibitem{Mixing}
R. C. Bradley, ``Basic properties of strong mixing conditions. A survey and some open questions,'' arXiv preprint math/0511078, 2005.

\bibitem{Geo}
P. Diaconis and D. Stroock,  ``Geometric bounds for eigenvalues of Markov chains,'' \textit{The Annals of Applied Probability}, pp.36-61, 1991.

\bibitem{bound}
H. J.  Landau and A. M. Odlyzko,  ``Bounds for eigenvalues of certain stochastic matrices,'' Linear algebra and its Applications, 38, pp.5-15, 1981. 
% \bibitem{Ioannidis}
% Stratis Ioannidis and Edmund Yeh, ``Adaptive Caching Networks with Optimality Guarantees.'' \textit{IEEE/ACM Transactions on Networking.} Vol. 26, No. 2, April 2018, pp. 737-750.

% \bibitem{composition}
% Kairouz, P., Oh, S. and P. Viswanath, ``The composition theorem for differential privacy,'' in \textit{Proc. Int. Conf. Machine Learning, PMLR,} pp. 1376-1385,  June 2015.

\bibitem{AR}
S. Cambanis and I. Fakhre-Zakeri,  ``Forward and reversed time prediction of autoregressive sequences,'' \textit{Journal of applied probability}, vol.  33, no. 4, pp.1053-1060, 1996.

% \bibitem{AoIPrivacy}
% R. Jin, X. He and H. Dai, ``Minimizing the Age of Information in the Presence of Location Privacy-Aware Mobile Agents,'' \textit{IEEE Transactions on Communications}, vol. 69, no. 2, pp. 1053-1067, Feb. 2021.

\bibitem{Bayes}
A. Triastcyn, 
B. Faltings, ``Bayesian Differential Privacy for Machine Learning,'' in \textit{Proc. International Conference on Machine Learning}, 2020.


\bibitem{MMSE}
D. Guo, S. Shamai, and S. Verdú,  ``Mutual information and minimum mean-square error in Gaussian channels,'' \textit{IEEE Trans. Inf. Theory}, 51(4), pp.1261-1282, 2005.

\bibitem{Ber}
Fintel, ``Berkshire Hathaway Inc - Filing History''. Avaiable: \url{https://fintel.io/i13fs/berkshire-hathaway}.

\bibitem{CVX}
 M. Grant, S. Boyd, and Y. Ye,  CVX: Matlab software for disciplined convex programming, 2009.

\bibitem{Boyd}
S. Boyd and L. Vandenberghe, Convex optimization. Cambridge university press,  2004.

\bibitem{Prob}
Stroock, Daniel W. Probability theory: an analytic view. Cambridge university press, 2010.

\bibitem{incorrect}
A. Maatouk, S.  Kriouile, M. Assaad, and A. Ephremides,  ``The age of incorrect information: A new performance metric for status updates,'' \textit{IEEE/ACM Trans. Netw.}, vol. 28, no. 5, pp.2215-2228, 2020.


\bibitem{London}
UK Power Networks, ``SmartMeter Energy Consumption Data in London Households,'' 2013. Available: \url{https://data.london.gov.uk/dataset/smartmeter-energy-use-data-in-london-households}



\end{thebibliography}
